The California-Kepler Survey. IV. Metal-rich Stars Host a Greater Diversity of Planets

Probing the connection between a star's metallicity and the presence and properties of any associated planets offers an observational link between conditions during the epoch of planet formation and mature planetary systems. We explore this connection by analyzing the metallicities of Kepler target stars and the subset of stars found to host transiting planets. After correcting for survey incompleteness, we measure planet occurrence: the number of planets per 100 stars with a given metallicity $M$. Planet occurrence correlates with metallicity for some, but not all, planet sizes and orbital periods. For warm super-Earths having $P = 10-100$ days and $R_P = 1.0-1.7~R_E$, planet occurrence is nearly constant over metallicities spanning $-$0.4 dex to +0.4 dex. We find 20 warm super-Earths per 100 stars, regardless of metallicity. In contrast, the occurrence of warm sub-Neptunes ($R_P = 1.7-4.0~R_E$) doubles over that same metallicity interval, from 20 to 40 planets per 100 stars. We model the distribution of planets as $d f \propto 10^{\beta M} d M$, where $\beta$ characterizes the strength of any metallicity correlation. This correlation steepens with decreasing orbital period and increasing planet size. For warm super-Earths $\beta = -0.3^{+0.2}_{-0.2}$, while for hot Jupiters $\beta = +3.4^{+0.9}_{-0.8}$. High metallicities in protoplanetary disks may increase the mass of the largest rocky cores or the speed at which they are assembled, enhancing the production of planets larger than 1.7 $R_E$. The association between high metallicity and short-period planets may reflect disk density profiles that facilitate the inward migration of solids or higher rates of planet-planet scattering.

==> tab_occurrence.tex <==
22.63 & 32.00 & 1.00 & 1.78 & 0 & 1.00 & 6906.2 & $< 0.03$ \\
22.63 & 32.00 & 1.78 & 3.16 & 0 & 1.00 & 4705.2 & $< 0.05$ \\
22.63 & 32.00 & 3.16 & 5.62 & 0 & 1.00 & 3205.6 & $< 0.07$ \\
22.63 & 32.00 & 5.62 & 10.00 & 0 & 1.00 & 2183.9 & $< 0.10$ \\
22.63 & 32.00 & 10.00 & 17.78 & 0 & 1.00 & 1487.9 & $< 0.15$ \\
22.63 & 32.00 & 17.78 & 31.62 & 0 & 1.00 & 1013.7 & $< 0.23$ \\
22.63 & 32.00 & 31.62 & 56.23 & 0 & 1.00 & 690.6 & $< 0.32$ \\
22.63 & 32.00 & 56.23 & 100.00 & 0 & 1.00 & 470.5 & $< 0.49$ \\
22.63 & 32.00 & 100.00 & 177.83 & 0 & 1.00 & 320.6 & $< 0.71$ \\
22.63 & 32.00 & 177.83 & 316.23 & 0 & 1.00 & 218.4 & $< 1.05$ \\
16.00 & 22.63 & 1.00 & 1.78 & 0 & 1.00 & 6906.2 & $< 0.03$ \\
16.00 & 22.63 & 1.78 & 3.16 & 0 & 1.00 & 4705.2 & $< 0.05$ \\
16.00 & 22.63 & 3.16 & 5.62 & 2 & 1.00 & 3205.6 & $0.08^{+0.06}_{-0.04}$ \\
16.00 & 22.63 & 5.62 & 10.00 & 0 & 1.00 & 2183.9 & $< 0.10$ \\
16.00 & 22.63 & 10.00 & 17.78 & 0 & 1.00 & 1487.9 & $< 0.16$ \\
16.00 & 22.63 & 17.78 & 31.62 & 0 & 1.00 & 1013.7 & $< 0.23$ \\
16.00 & 22.63 & 31.62 & 56.23 & 0 & 1.00 & 690.6 & $< 0.34$ \\
16.00 & 22.63 & 56.23 & 100.00 & 0 & 1.00 & 470.5 & $< 0.47$ \\
16.00 & 22.63 & 100.00 & 177.83 & 0 & 1.00 & 320.6 & $< 0.71$ \\
16.00 & 22.63 & 177.83 & 316.23 & 0 & 1.00 & 218.4 & $< 1.03$ \\
11.31 & 16.00 & 1.00 & 1.78 & 1 & 1.00 & 6906.2 & $0.02^{+0.02}_{-0.01}$ \\
11.31 & 16.00 & 1.78 & 3.16 & 3 & 1.00 & 4705.2 & $0.08^{+0.05}_{-0.03}$ \\
11.31 & 16.00 & 3.16 & 5.62 & 6 & 1.00 & 3205.6 & $0.21^{+0.09}_{-0.07}$ \\
11.31 & 16.00 & 5.62 & 10.00 & 1 & 1.00 & 2183.9 & $0.08^{+0.07}_{-0.04}$ \\
11.31 & 16.00 & 10.00 & 17.78 & 0 & 1.00 & 1487.9 & $< 0.15$ \\
11.31 & 16.00 & 17.78 & 31.62 & 0 & 1.00 & 1013.7 & $< 0.23$ \\
11.31 & 16.00 & 31.62 & 56.23 & 1 & 1.00 & 690.6 & $0.24^{+0.23}_{-0.14}$ \\
11.31 & 16.00 & 56.23 & 100.00 & 0 & 1.00 & 470.5 & $< 0.49$ \\
11.31 & 16.00 & 100.00 & 177.83 & 1 & 1.00 & 320.5 & $0.52^{+0.51}_{-0.30}$ \\
11.31 & 16.00 & 177.83 & 316.23 & 1 & 1.00 & 218.4 & $0.77^{+0.73}_{-0.44}$ \\
8.00 & 11.31 & 1.00 & 1.78 & 0 & 1.00 & 6906.2 & $< 0.03$ \\
8.00 & 11.31 & 1.78 & 3.16 & 0 & 1.00 & 4705.1 & $< 0.05$ \\
8.00 & 11.31 & 3.16 & 5.62 & 1 & 1.00 & 3205.5 & $0.05^{+0.05}_{-0.03}$ \\
8.00 & 11.31 & 5.62 & 10.00 & 0 & 1.00 & 2183.8 & $< 0.11$ \\
8.00 & 11.31 & 10.00 & 17.78 & 0 & 1.00 & 1487.8 & $< 0.15$ \\
8.00 & 11.31 & 17.78 & 31.62 & 2 & 1.00 & 1013.6 & $0.26^{+0.20}_{-0.13}$ \\
8.00 & 11.31 & 31.62 & 56.23 & 1 & 1.00 & 690.6 & $0.24^{+0.23}_{-0.14}$ \\
8.00 & 11.31 & 56.23 & 100.00 & 0 & 1.00 & 470.4 & $< 0.48$ \\
8.00 & 11.31 & 100.00 & 177.83 & 4 & 1.00 & 320.4 & $1.45^{+0.75}_{-0.56}$ \\
8.00 & 11.31 & 177.83 & 316.23 & 5 & 1.00 & 218.3 & $2.59^{+1.21}_{-0.92}$ \\
5.66 & 8.00 & 1.00 & 1.78 & 0 & 1.00 & 6905.9 & $< 0.03$ \\
5.66 & 8.00 & 1.78 & 3.16 & 0 & 1.00 & 4704.9 & $< 0.05$ \\
5.66 & 8.00 & 3.16 & 5.62 & 1 & 1.00 & 3205.3 & $0.05^{+0.05}_{-0.03}$ \\
5.66 & 8.00 & 5.62 & 10.00 & 2 & 1.00 & 2183.7 & $0.12^{+0.09}_{-0.06}$ \\
5.66 & 8.00 & 10.00 & 17.78 & 2 & 1.00 & 1487.6 & $0.18^{+0.13}_{-0.09}$ \\
5.66 & 8.00 & 17.78 & 31.62 & 1 & 1.00 & 1013.4 & $0.17^{+0.16}_{-0.10}$ \\
5.66 & 8.00 & 31.62 & 56.23 & 2 & 1.00 & 690.2 & $0.38^{+0.28}_{-0.19}$ \\
5.66 & 8.00 & 56.23 & 100.00 & 0 & 1.00 & 470.0 & $< 0.49$ \\
5.66 & 8.00 & 100.00 & 177.83 & 0 & 1.00 & 319.9 & $< 0.70$ \\
5.66 & 8.00 & 177.83 & 316.23 & 3 & 0.99 & 217.6 & $1.68^{+1.01}_{-0.72}$ \\
4.00 & 5.66 & 1.00 & 1.78 & 0 & 1.00 & 6905.3 & $< 0.03$ \\
4.00 & 5.66 & 1.78 & 3.16 & 0 & 1.00 & 4704.2 & $< 0.05$ \\
4.00 & 5.66 & 3.16 & 5.62 & 3 & 1.00 & 3204.5 & $0.12^{+0.07}_{-0.05}$ \\
4.00 & 5.66 & 5.62 & 10.00 & 1 & 1.00 & 2182.7 & $0.08^{+0.07}_{-0.04}$ \\
4.00 & 5.66 & 10.00 & 17.78 & 3 & 1.00 & 1486.3 & $0.25^{+0.15}_{-0.11}$ \\
4.00 & 5.66 & 17.78 & 31.62 & 5 & 1.00 & 1011.7 & $0.56^{+0.26}_{-0.20}$ \\
4.00 & 5.66 & 31.62 & 56.23 & 3 & 0.99 & 688.2 & $0.53^{+0.31}_{-0.23}$ \\
4.00 & 5.66 & 56.23 & 100.00 & 3 & 0.99 & 467.7 & $0.78^{+0.48}_{-0.34}$ \\
4.00 & 5.66 & 100.00 & 177.83 & 2 & 0.99 & 317.4 & $0.84^{+0.62}_{-0.41}$ \\
4.00 & 5.66 & 177.83 & 316.23 & 1 & 0.98 & 214.9 & $0.78^{+0.76}_{-0.45}$ \\
2.83 & 4.00 & 1.00 & 1.78 & 0 & 1.00 & 6901.8 & $< 0.03$ \\
2.83 & 4.00 & 1.78 & 3.16 & 2 & 1.00 & 4700.0 & $0.06^{+0.04}_{-0.03}$ \\
2.83 & 4.00 & 3.16 & 5.62 & 2 & 1.00 & 3199.4 & $0.08^{+0.06}_{-0.04}$ \\
2.83 & 4.00 & 5.62 & 10.00 & 20 & 1.00 & 2176.7 & $0.94^{+0.22}_{-0.19}$ \\
2.83 & 4.00 & 10.00 & 17.78 & 26 & 0.99 & 1479.6 & $1.80^{+0.36}_{-0.32}$ \\
2.83 & 4.00 & 17.78 & 31.62 & 18 & 0.99 & 1004.4 & $1.85^{+0.46}_{-0.39}$ \\
2.83 & 4.00 & 31.62 & 56.23 & 17 & 0.98 & 680.5 & $2.58^{+0.66}_{-0.57}$ \\
2.83 & 4.00 & 56.23 & 100.00 & 12 & 0.97 & 459.5 & $2.75^{+0.83}_{-0.68}$ \\
2.83 & 4.00 & 100.00 & 177.83 & 9 & 0.96 & 308.7 & $3.12^{+1.09}_{-0.87}$ \\
2.83 & 4.00 & 177.83 & 316.23 & 4 & 0.94 & 205.8 & $2.25^{+1.17}_{-0.88}$ \\
2.00 & 2.83 & 1.00 & 1.78 & 0 & 0.99 & 6882.1 & $< 0.03$ \\
2.00 & 2.83 & 1.78 & 3.16 & 3 & 0.99 & 4678.6 & $0.08^{+0.05}_{-0.03}$ \\
2.00 & 2.83 & 3.16 & 5.62 & 24 & 0.99 & 3176.6 & $0.77^{+0.17}_{-0.14}$ \\
2.00 & 2.83 & 5.62 & 10.00 & 29 & 0.98 & 2152.4 & $1.38^{+0.26}_{-0.23}$ \\
2.00 & 2.83 & 10.00 & 17.78 & 61 & 0.98 & 1454.1 & $4.23^{+0.54}_{-0.51}$ \\
2.00 & 2.83 & 17.78 & 31.62 & 48 & 0.96 & 978.3 & $4.97^{+0.72}_{-0.64}$ \\
2.00 & 2.83 & 31.62 & 56.23 & 43 & 0.95 & 654.2 & $6.67^{+1.01}_{-0.93}$ \\
2.00 & 2.83 & 56.23 & 100.00 & 20 & 0.92 & 433.4 & $4.75^{+1.11}_{-0.95}$ \\
2.00 & 2.83 & 100.00 & 177.83 & 7 & 0.88 & 282.9 & $2.70^{+1.06}_{-0.83}$ \\
2.00 & 2.83 & 177.83 & 316.23 & 2 & 0.82 & 180.7 & $1.47^{+1.05}_{-0.72}$ \\
1.41 & 2.00 & 1.00 & 1.78 & 5 & 0.98 & 6801.0 & $0.08^{+0.04}_{-0.03}$ \\
1.41 & 2.00 & 1.78 & 3.16 & 15 & 0.97 & 4593.0 & $0.34^{+0.09}_{-0.08}$ \\
1.41 & 2.00 & 3.16 & 5.62 & 38 & 0.96 & 3092.1 & $1.25^{+0.21}_{-0.19}$ \\
1.41 & 2.00 & 5.62 & 10.00 & 41 & 0.95 & 2073.3 & $2.02^{+0.31}_{-0.30}$ \\
1.41 & 2.00 & 10.00 & 17.78 & 38 & 0.92 & 1379.5 & $2.79^{+0.46}_{-0.42}$ \\
1.41 & 2.00 & 17.78 & 31.62 & 23 & 0.89 & 904.9 & $2.61^{+0.58}_{-0.49}$ \\
1.41 & 2.00 & 31.62 & 56.23 & 14 & 0.84 & 580.0 & $2.51^{+0.70}_{-0.58}$ \\
1.41 & 2.00 & 56.23 & 100.00 & 6 & 0.76 & 359.1 & $1.86^{+0.77}_{-0.62}$ \\
1.41 & 2.00 & 100.00 & 177.83 & 7 & 0.66 & 211.8 & $3.60^{+1.39}_{-1.14}$ \\
1.41 & 2.00 & 177.83 & 316.23 & 4 & 0.53 & 117.3 & $3.93^{+2.04}_{-1.52}$ \\
1.00 & 1.41 & 1.00 & 1.78 & 7 & 0.95 & 6551.6 & $0.12^{+0.05}_{-0.04}$ \\
1.00 & 1.41 & 1.78 & 3.16 & 15 & 0.93 & 4369.1 & $0.36^{+0.10}_{-0.08}$ \\
1.00 & 1.41 & 3.16 & 5.62 & 40 & 0.89 & 2874.8 & $1.41^{+0.23}_{-0.21}$ \\
1.00 & 1.41 & 5.62 & 10.00 & 48 & 0.84 & 1847.5 & $2.63^{+0.39}_{-0.36}$ \\
1.00 & 1.41 & 10.00 & 17.78 & 51 & 0.76 & 1144.3 & $4.50^{+0.64}_{-0.59}$ \\
1.00 & 1.41 & 17.78 & 31.62 & 23 & 0.66 & 673.5 & $3.50^{+0.76}_{-0.65}$ \\
1.00 & 1.41 & 31.62 & 56.23 & 10 & 0.53 & 370.5 & $2.87^{+0.95}_{-0.78}$ \\
1.00 & 1.41 & 56.23 & 100.00 & 4 & 0.39 & 187.4 & $2.49^{+1.26}_{-0.97}$ \\
1.00 & 1.41 & 100.00 & 177.83 & 0 & 0.27 & 86.4 & $< 2.61$ \\
1.00 & 1.41 & 177.83 & 316.23 & 0 & 0.16 & 36.3 & $\nodata$ \\
0.71 & 1.00 & 1.00 & 1.78 & 6 & 0.84 & 5809.6 & $0.12^{+0.05}_{-0.04}$ \\
0.71 & 1.00 & 1.78 & 3.16 & 18 & 0.76 & 3574.6 & $0.52^{+0.13}_{-0.11}$ \\
0.71 & 1.00 & 3.16 & 5.62 & 26 & 0.64 & 2081.1 & $1.28^{+0.26}_{-0.23}$ \\
0.71 & 1.00 & 5.62 & 10.00 & 35 & 0.51 & 1130.2 & $3.15^{+0.54}_{-0.49}$ \\
0.71 & 1.00 & 10.00 & 17.78 & 11 & 0.38 & 566.1 & $2.05^{+0.66}_{-0.54}$ \\
0.71 & 1.00 & 17.78 & 31.62 & 11 & 0.25 & 259.9 & $4.47^{+1.39}_{-1.17}$ \\
0.71 & 1.00 & 31.62 & 56.23 & 2 & 0.15 & 109.0 & $\nodata$ \\
0.71 & 1.00 & 56.23 & 100.00 & 1 & 0.09 & 41.7 & $\nodata$ \\
0.71 & 1.00 & 100.00 & 177.83 & 0 & 0.04 & 14.6 & $\nodata$ \\
0.71 & 1.00 & 177.83 & 316.23 & 0 & 0.02 & 4.7 & $\nodata$ \\
0.50 & 0.71 & 1.00 & 1.78 & 2 & 0.48 & 3371.8 & $0.08^{+0.06}_{-0.04}$ \\
0.50 & 0.71 & 1.78 & 3.16 & 9 & 0.35 & 1651.3 & $0.58^{+0.21}_{-0.17}$ \\
0.50 & 0.71 & 3.16 & 5.62 & 13 & 0.23 & 743.7 & $\nodata$ \\
0.50 & 0.71 & 5.62 & 10.00 & 7 & 0.14 & 309.3 & $\nodata$ \\
0.50 & 0.71 & 10.00 & 17.78 & 2 & 0.08 & 119.6 & $\nodata$ \\
0.50 & 0.71 & 17.78 & 31.62 & 1 & 0.04 & 43.2 & $\nodata$ \\
0.50 & 0.71 & 31.62 & 56.23 & 0 & 0.02 & 14.5 & $\nodata$ \\
0.50 & 0.71 & 56.23 & 100.00 & 0 & 0.01 & 4.5 & $\nodata$ \\
0.50 & 0.71 & 100.00 & 177.83 & 0 & 0.00 & 1.2 & $\nodata$ \\
0.50 & 0.71 & 177.83 & 316.23 & 0 & 0.00 & 0.3 & $\nodata$ \\
